Testing Models of Strategic Uncertainty: Equilibrium Selection in Repeated Games

In repeated-game applications where both the collusive and non-collusive outcomes can be supported as equilibria, researchers must resolve underlying selection questions if theory will be used to understand counterfactual policies. One guide to selection, based on clear theoretical underpinnings, has shown promise in predicting when collusive outcomes will emerge in controlled repeated-game experiments. In this paper we both expand upon and experimentally test this model of selection, and its underlying mechanism: strategic uncertainty. Adding an additional source of strategic uncertainty (the number of players) to the more-standard payoff sources, we stress test the model. Our results affirm the model as a tool for predicting when tacit collusion is likely/unlikely to be successful. Extending the analysis, we corroborate the mechanism of the model. When we remove strategic uncertainty through an explicit coordination device, the model no longer predicts the selected equilibrium.

==> bin/oldIntro.tex <==


%Our paper examines the predictive power of the basin for equilibrium selection over the number of participants. We design a $2\times2$ between-subject test that uses independence across players to generalize the basin notion, where in one dimension we vary the basin prediction, while in the other we hold constant the basin prediction but vary the prediction under a null hypothesis of no-response to $N$. While our results for initial cooperation rates show more mixed evidence, in terms of successful, ongoing coordination on the PM-SPE, the basin prediction from repeated PD-games is predictive both qualitatively, and quantitatively.

%We then examine two further checks. In the first, we change the identification strategy. Rather than a comparison of the equilibrium-selection effects across separate populations at differing $N$, we instead compare a change in $N$ within population. The shift in identification attempts to create a clearer parallel to a policy change within a population, one that has already converged to one equilibria or another. Assessing the idea that a specific equilibrium may be sticky within a particular population, our data here mirrors the results from our between-population analysis. In fact, if anything the results within are even starker, with participants moving from large to small $N$ showing an immediate and large jump in collusive play as soon as the change happens.

%Finally, we examine the effects from explicit collusion, where treating players as independently deciding whether to collude or not will clearly be a stretch. Under the harshest parameter set for implicit collusion, where we get less than 1 percent ongoing attempts at collusion, the provision of preplay chat to the group shifts behavior toward the opposite extreme, with over 75 percent of groups successfully colluding. The treatment therefore both serves as both a sanity check on the necessity of anti-collusion laws such as the Sherman Act, but as a clear identification that strategic uncertainty is a primary driver of selection. However, in a parallel treatment we show that there are limits on what explicit collusion can achieve. Holding constant $N$ and the stage-game, we lower the discount rate to the point where collusion is a knife-edge equilibrium. Where an explicit collusion achieves 75 percent ongoing success with the higher discount, when theoretically knife-edge, the ongoing success rate falls to near zero (0.2 percent).





%More broadly, we would like to assess to what extent equilibrium selection in a social-dilemma setting can be associated with strategic uncertainty. From the RPD we know that modifying the temptation parameter changes $p^{\star}$: A lower temptation to deviate from cooperation reduces $p^{\star}$, and predicts that cooperation will be easier. But if what determines equilibrium selection are difficulties to coordinate, then increasing the number of players $N$ should compensate in the opposite direction in the sense that more players presumably increase strategic uncertainty. Assessing strategic uncertainty by changing $N$ is not feasible within the RPD, as changing $N$ (or several other variables that are important in counterfactuals) is not possible. Because changing $N$ is often deemed as crucial for collusion practices, we evaluate to what

%that a criterion for equilibrium selection can be of useful for assessing counterfactuals, consider the following stylized interpretation of our main treatment variation. A symmetric group of $N$ firms are competing in a repeated Bertrand environment. The model primitives are textbook, with linear market demand given by $Q(p)=A-p$, where firms have constant marginal costs given by $c>0$. Firms are pushing for consolidation-friendly policy, where they can convincingly argue that efficiency gains from increased market share will push down their marginal costs. Two focal theoretic outcomes here are: (i) the stationary non-collusive outcome (the Markov Perfect Equilibrium, MPE) where firms price at $p^\star=c$; and (ii) a collusive outcome of $p^\star=\nicefrac{1}{2}\cdot(A+c)$ supported by the threat of a price war (if discount-rates are high enough, the profit-maximizing sub-game perfect outcome PM-SPE). 

%To motivate the idea that a criterion for equilibrium selection can be of useful for assessing counterfactuals, consider the following stylized interpretation of our main treatment variation. A symmetric group of $N$ firms are competing in a repeated Bertrand environment. The model primitives are textbook, with linear market demand given by $Q(p)=A-p$, where firms have constant marginal costs given by $c>0$. Firms are pushing for consolidation-friendly policy, where they can convincingly argue that efficiency gains from increased market share will push down their marginal costs. Two focal theoretic outcomes here are: (i) the stationary non-collusive outcome (the Markov Perfect Equilibrium, MPE) where firms price at $p^\star=c$; and (ii) a collusive outcome of $p^\star=\nicefrac{1}{2}\cdot(A+c)$ supported by the threat of a price war (if discount-rates are high enough, the profit-maximizing sub-game perfect outcome PM-SPE). 

%Considering a counterfactual decrease in the number of firms, constant assumption of the MPE suggests a consolidation price-effect of $\Delta p^\star=\Delta c<0$. In contrast, constant assumption of the PM-SPE (and assuming  demand $A$ is unaffected) predicts a price change of $\Delta p^\star=\nicefrac{1}{2}\cdot\Delta c<0$. Under this model, while the two equilibria differ in the quantitative benefits to consumers, constant selection of each lead to the same policy conclusion: consolidation (up to two firms) is in the interest of consumers. However, if equilibrium selection is instead a function of the policy variable $N$, then this conclusion can be reversed. If collusion becomes easier to coordinate on with a smaller number of firms, and the selected equilibria changes with the policy variable, it is instead possible that prices increase by $\Delta p^\star=\nicefrac{1}{2}\cdot(A-c-\Delta c)$.





%from a policy change---one  response to the problem is to hold constant the selection assumption. A stronger variant of this approach would be to consider the policy-relevant comparative static across a number of focal equilibria. 

%The equilibrium selection notion that has become focal in this literature is based on the ideas of risk-dominance and the basin of attraction---a theoretical literature going back to \citeauthor{harsanyi1988general}. One strength of this notion (as opposed to more reduced-form fits) is that it can be readily generalized. This strength forms a complement to a weakness in the data identifying the basin's predictive power: that it examines a stylized two-player environment. In this paper, we examine a generalization of the basin to an $N$-player setting. While we maintain many other stark features of the repeated PD environment, our experiments isolate and tests how a generalization of the PD-identified basin functions as both a qualitative and quantitative predictor of selection as we move out-of-context.


%Points to make: 
%1. Counterfactuals often involve changes in two variables at the same time, not just changing N.
%2. Strategic uncertainty as an idea to think of equilibrium selection.
%3. Communication shows that it's not about trust that it is about coordination (provided that collusion is an SPE, that is, that incentives are there).

%Mirroring the above example, our experiments outline exactly this pattern. Though the profit-maximizing and stationary outcomes are both supportable as equilibria across all of our treatments, participants readily coordinate on the PM-SPE when the number of players is small, and on the MPE when the number of players is large. However, their success at coordinating on the PM-MPE is well-predicted, both qualitatively and quantitatively, by a simple generalization of the basin of attraction concept. 

%Our environment is obviously still highly stylized, and readers from fields such as IO are probably leery of reading too much into a single lab experiment. However, the stakes here are large enough that some optimism for a simple, extensible selection criterion is warranted. Theory for ongoing environments with ongoing with long-run actors---represented by Folk Theorems of various stripes---demonstrates how unavoidable selection questions are in settings of interest. While extant data can help us address equilibrium selection question under the status quo, as we move into the unknown of a counterfactual policy we must act under some maintained belief. Extensions of the basin of attraction offer a simple theoretical device backed by a substantial empirically based literature, to examine the plausibility of differential equilibrium selection as we shift policy levers.

==> tab/TreatmentSimpleOngoing.tex <==
\begin{tabular}{cccccc}\toprule
 \multirow[c]{2}{*}{\minitab[c]{\bf Stage-game \\\bf payoffs}}   & \multicolumn{2}{c}{$x=\$9$} & &\multicolumn{2}{c}{$x=\$1$}\\ \cmidrule{2-3}\cmidrule{5-6}
  %$u_i\left(a_i,\sigma\right)$ 
  & $\sigma(a_{-i})=S$ & $\sigma(a_{-i})=F$ & & $\sigma(a_{-i})=S$ & $\sigma(a_{-i})=F$ \\ \midrule
  Coop., $u_i(C,\sigma)$ & $\$20$ & $\$2$ &  &  $\$20$ & $\$10$ \\
  Defect, $u_i(C,\sigma)$ & $\$29$ & $\$11$ & &  $\$21$ & $\$11$ \\ \midrule
 \multirow[c]{2}{*}{\minitab[c]{\bf Experimental \\\bf variables}} & \multicolumn{2}{c}{$x=\$9$} & &\multicolumn{2}{c}{$x=\$1$}\\ \cmidrule{2-3}\cmidrule{5-6}
 & $N=2$ & $N=4$ & & $N=4$ & $N=10$ \\ \midrule
Cor. basin, $p^{\star}_{\text{Cor.}}(x)$ & $p^\star_0$ & $p^\star_0$&  & $p^\star_0-\Delta p^\star_{\text{Cor.}}$ & $p^\star_0-\Delta p^\star_{\text{Cor.}}$\\

& [0.333] & [0.333] & & [0.037] & [0.037] \\
  
Ind. basin, $p^{\star}_{\text{Ind.}}(x,N)$ 
& $p^\star_0$ & $p^\star_0+\Delta p^\star_{\text{Ind.}}$&  & $p^\star_0$ & $p^\star_0+\Delta p^\star_{\text{Ind.}}$\\
& [0.333] & [0.693] & & [0.333] & [0.693] \\
\cmidrule{2-6}
Sessions        & 3  & 3 & & 3 & 3 \\
Subjects        & 60 & 60 & & 72 & 60 \\  
\midrule
\multicolumn{6}{l}{\textbf{Panel C}} \\
\multirow[c]{2}{*}{\minitab[c]{\bf Meta-study \\\bf predictions}} & $p^\star_0$  &  \multicolumn{4}{c}{\hspace{0.2in}$\Delta$Coop. on basis size change:} \\ \cmidrule{3-6}

&  & \multicolumn{3}{c}{$-\Delta p^\star_{\text{Cor.}}$} & $+\Delta p^\star_{\text{Ind.}}$ \\ \midrule
Initial coop.& 0.495  & \multicolumn{3}{c}{+0.345}  & -0.258   \\
($t=1$) & \SD{0.037} & \multicolumn{3}{c}{\SD{0.070}}& \SD{0.036}  \\
 Ongoing coop. & 0.373 & \multicolumn{3}{c}{+0.347}  & -0.211  \\ 
($t>1$) & \SD{0.035} & \multicolumn{3}{c}{\SD{0.066}}& \SD{0.026}  \\ \bottomrule 
\end{tabular}
\begin{tablenotes}  Meta-study prediction indicates the cooperation rate predictions from the 2-player basin (with standard errors in parentheses) recovered from treatment-clustered probits, using the specifications illustrated in Figure \ref{fig:MetaStudy}.
\end{tablenotes}

==> tab/archive/CoopTable.tex <==
\begin{tabular}{ccccccccc}
\toprule  & \multicolumn{8}{c}{Cooperation Rates}\\ 
\cmidrule{2-9} & \multicolumn{2}{c}{Individual ($t=1$)} &  & \multicolumn{2}{c}{Joint ($t=1$)} &  & \multicolumn{2}{c}{Ongoing ($t>1$)}\\ 
\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9} & $p_{L}^{\star}$ & $p_{H}^{\star}$ &  & $p_{L}^{\star}$ & $p_{H}^{\star}$ &  & $p_{L}^{\star}$ & $p_{H}^{\star}$\\ 
\midrule $x_{L}$ & 0.792 & 0.357 &  & 0.511 & 0 &  & 0.409 & 0.185\\ 
 & \SD{0.042} & \SD{0.055} &  & \SD{0.053} & \SD{-} &  & \SD{0.050} & \SD{0.048}\\ 
$x_{H}$ & 0.503 & 0.035 &  & 0.280 & 0 &  & 0.450 & 0.006\\ 
 & \SD{0.058} & \SD{0.017} &  & \SD{0.037} & \SD{-} &  & \SD{0.055} & \SD{0.003}\\ \midrule & \multicolumn{8}{c}{Regression decomposition}\\ 
\cmidrule{2-9}
Ind. Basin: $\Delta p^\star_{\text{Ind}}$ & \multicolumn{2}{c}{-0.451} &  & \multicolumn{2}{c}{-0.357} &  & \multicolumn{2}{c}{-0.325}\\ 
 & \multicolumn{2}{c}{\SD{0.046}} &  & \multicolumn{2}{c}{\SD{0.049}} &  & \multicolumn{2}{c}{\SD{0.047}}\\ 
Corr. Basin: $\Delta\tilde{p}_{\text{Corr}}$ & \multicolumn{2}{c}{-0.304} &  & \multicolumn{2}{c}{-0.169} &  & \multicolumn{2}{c}{-0.068}\\ 
 & \multicolumn{2}{c}{\SD{0.047}} &  & \multicolumn{2}{c}{\SD{0.046}} &  & \multicolumn{2}{c}{\SD{0.046}}\\ 
\midrule Obs. & \multicolumn{2}{c}{$1,220$} &  & \multicolumn{2}{c}{$335$} &  & \multicolumn{2}{c}{$2,892$}\\ \bottomrule 
\end{tabular}
\begin{tablenotes}
Standard errors in parentheses, for \emph{Individual} and \emph{Ongoing} these are clustered at the subject level. Cooperation-rate standard errors are recovered from bernoulli-exact confidence intervals on proportion rests. Regression-decomposition standard errors from a linear-probability model.
\end{tablenotes}




==> tab/archive/CoopTableAlt.tex <==
\begin{tabular}{cccccc}
\multicolumn{6}{l}{\emph{(A) Experiment cooperation rates}} \\ 
\toprule
 & \multicolumn{2}{c}{Individual ($t=1$)} &   & \multicolumn{2}{c}{Ongoing ($t>1$)}\\ 
 \cmidrule{2-3}\cmidrule{5-6}
Corr/Ind Basin & $p^\star=p_0$ & $p^\star=p_0+\Delta p_{\text{Ind.}}$ &  & $p_0$ & $p_0+\Delta p^\star_{\text{Ind.}}$\\ 
\midrule 
    $\tilde{p}=p_0$ & 0.503 & 0.035 &  & 0.450 & 0.006\\ 
       & \SD{0.058} & \SD{0.017} &  & \SD{0.055} & \SD{0.003}\\
  $\tilde{p}=p_0-\Delta \tilde{p}_{\text{Cor.}}$ & 0.792 & 0.357 &  & 0.409 & 0.185\\ 
 & \SD{0.042} & \SD{0.055} &  & \SD{0.050} & \SD{0.048}\\ \bottomrule
 \\
 \multicolumn{5}{l}{\emph{(B) Effect decomposition}}\\ 
\toprule 
& \multicolumn{2}{c}{Individual ($t=1$)} &   & \multicolumn{2}{c}{Ongoing ($t>1$)}\\
\midrule
Ind. Basin: $\Delta p^\star_{\text{Ind}}$ & 
   \multicolumn{2}{c}{-0.434}     & & \multicolumn{2}{c}{-0.402}\\ 
 & \multicolumn{2}{c}{\SD{0.074}} & & \multicolumn{2}{c}{\SD{0.072}}\\ 
Corr. Basin: $-\Delta\tilde{p}_{\text{Corr}}$ & 
   \multicolumn{2}{c}{0.257}     & & \multicolumn{2}{c}{-0.027}\\ 
 & \multicolumn{2}{c}{\SD{0.088}} & & \multicolumn{2}{c}{\SD{0.103}}\\ 
\midrule Obs. & \multicolumn{2}{c}{$1,220$} &  & \multicolumn{2}{c}{$2,892$}\\ \bottomrule 

\end{tabular}
\begin{tablenotes}
Standard errors in parentheses clustered at the subject level. Cooperation-rate figures standard errors recovered from bernoulli-exact confidence intervals on proportion rests. Effect decomposition estimates and standard errors from a subject-clustered probit model.
\end{tablenotes}

==> tab/archive/TreatmentTable.tex <==
\subfloat[$x=1$]{\centering
\begin{tabular}{p{0.1in}c|c|c|}
   & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Outcome,  $\sigma(a_{-i})$}\\  \cmidrule{3-4}
   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Success} & \multicolumn{1}{c}{Failure}\\ 
\cline{3-4} \cline{4-4} 
 \multirow{2}{*}{$a_{i}$:} & $C$ & $20$ & $10$\\ 
\cline{3-4} \cline{4-4} 
  & $D$ & $21$ & $11$\\ 
\cline{3-4} \cline{4-4} 
\end{tabular}
}
\subfloat[$x=9$]{\centering
\begin{tabular}{p{0.1in}c|c|c|}
   & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Outcome,  $\sigma(a_{-i})$}\\ \cmidrule{3-4}
   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Success} & \multicolumn{1}{c}{Failure}\\ 
\cline{3-4} \cline{4-4} 
 \multirow{2}{*}{$a_{i}$:}  & $C$ & $20$ & $2$\\ 
\cline{3-4} \cline{4-4} 
  & $D$ & $29$ & $11$\\ 
\cline{3-4} \cline{4-4} 
\end{tabular}
}

% \subfloat[Meta-study prediction (initial)]{\centering
% \begin{tabular}{lrc|c}
% &   & \multicolumn{2}{c}{Indep. Basin:} \\ %\cmidrule{3-4}
% &   & \multicolumn{1}{c}{$N(x,p_L)$} & $N(x,p_H)$ \\ 
%  \cline{3-4} \cline{4-4} 
% \multirow{2}{*}{Corr. Basin:} &  \multicolumn{1}{c|}{$x=9$} &  0.495 & \multicolumn{1}{c|}{ 0.237 }  \\
% \cline{3-4} \cline{4-4}
% &  \multicolumn{1}{c|}{
% $x=1$} &  0.843  & \multicolumn{1}{c|}{--} \\ 
% \cline{3-4} \cline{4-4}
% \end{tabular}
% }

% \subfloat[High Tempt. game, $x=9$]{\centering
% \begin{tabular}{lrc|c}
% &   & \multicolumn{2}{c}{Indep. Basin:} \\ %\cmidrule{3-4}
% &   & \multicolumn{1}{c}{$p^\star$} & $p^\star+\Delta p_{\text{Ind}}$ \\ 
%  \cline{3-4} \cline{4-4} 
% \multirow{2}{*}{Corr. Basin:} &  \multicolumn{1}{c|}{$p^\star$} &  0.373 & \multicolumn{1}{c|}{ 0.163 }  \\
% \cline{3-4} \cline{4-4}
% &  \multicolumn{1}{c|}{
% $p^\star-\Delta p_{\text{Corr}}$} &  0.718  & \multicolumn{1}{c|}{--} \\ 
% \cline{3-4} \cline{4-4}
% \end{tabular}}

